How to use the Standard Model effective field theory

We present a practical three-step procedure of using the Standard Model effective field theory (SM EFT) to connect ultraviolet (UV) models of new physics with weak scale precision observables. With this procedure, one can interpret precision measurements as constraints on a given UV model. We give a detailed explanation for calculating the effective action up to one-loop order in a manifestly gauge covariant fashion. This covariant derivative expansion method dramatically simplifies the process of matching a UV model with the SM EFT, and also makes available a universal formalism that is easy to use for a variety of UV models. A few general aspects of RG running effects and choosing operator bases are discussed. Finally, we provide mapping results between the bosonic sector of the SM EFT and a complete set of precision electroweak and Higgs observables to which present and near future experiments are sensitive. Many results and tools which should prove useful to those wishing to use the SM EFT are detailed in several appendices.

==> bk_sec_cde_examples.tex <==

In this subsection, we give several example models where we calculate the effective action using the covariant derivative expansion. As we will explicitly see, computing the Wilson coefficients for a given model proceeds in an essentially algorithmic fashion. If there is a tree-level contribution to the effective action, we use Eq.~\eqref{eqn:tree_cde_terms}. For the one-loop contribution, we use Eq.~\eqref{eqn:CDE_universal_lag}. Given a model, the brunt of the work is to identify the appropriate \(U\) to plug into Eqs.~\eqref{eqn:tree_cde_terms} and~\eqref{eqn:CDE_universal_lag} and then to evaluate the traces in these equations. In the following matching calculations, it should be understood that all the Wilson coefficients obtained are at the matching scale $\Lambda$, namely that all our results are actually about $c_i(\Lambda)$. That said, throughout this subsection we drop the specification of RG scale.

A note on terminology. We frequently, and somewhat inappropriately, refer to the use of Eqs.~\eqref{eqn:tree_cde_terms} and~\eqref{eqn:CDE_universal_lag} as ``using the CDE''. If we are just using the results in these equations, then such a statement is technically incorrect. The expansion of the effective action in these two equations can be obtained from \textit{any} consistent method to compute the effective action. The CDE is a \textit{particular} method which considerably eases obtaining these results, but, nevertheless, is still just a means to the end. With this clarification, we hope the reader can forgive our sloppy language in this section.

In demonstrating how to use the CDE to compute the effective action, we would also like to pick models that are of phenomenological interest. As such, we focus on models that couple to the bosonic sector of the SM, with particular attention towards those models which generate tree-level Wilson coefficients. UV models that generate tree-level Wilson coefficients of the bosonic operators in Table~\ref{tbl:operators} may substantially contribute to precision observables. As a result, these models are typically either already tightly constrained or will be probed in future. Note that RG running may be of practical relevance when the Wilson coefficient is generated at tree-level (see the discussion in section~\ref{sec:operatorbasis}). 

With the above motivations, we would like to make a list of possible UV models that have tree-level contributions to the effective action. Let us limit this list to heavy scalars which can couple at tree-level to the Higgs sector via renormalizable interactions. There are only four such theories:
% We limit this to theories where (1) the UV model is renormalizable and (2) the heavy field that we integrate out \textit{only couples with the bosonic fields of the SM}. There are only five such theories:
%If we require the UV model to be renormalizable and that the heavy field being integrated out \textit{only couples with the bosonic fields of the SM}, it turns out that there are only five of them:}

\begin{enumerate}
  \item A real singlet scalar $\Phi$
  \begin{equation}
  \Delta \mathcal{L} \supset \Phi \left|H\right|^2 .
  \end{equation}

  \item A real (complex) $SU(2)_L$ triplet scalar $\Phi_0=\Phi_0^a\tau^a$ ($\Phi_1=\Phi_1^a\tau^a$) with hypercharge $Y_\Phi=0$ ($Y_\Phi=1$)
  \begin{eqnarray}
  \Delta \mathcal{L} &\supset& H^\dagger \Phi_0 H , \\
  \Delta \mathcal{L} &\supset& H^\dagger \Phi_1 {\tilde H} +c.c. ,
  \end{eqnarray}
  where ${\tilde H}=i\sigma^2 H^*$.

  \item A complex $SU(2)_L$ doublet scalar $\Phi$ with $U(1)_Y$ hypercharge $Y_\Phi=\frac{1}{2}$
  \begin{equation}
  \Delta \mathcal{L} \supset \left|H\right|^2 (\Phi^\dagger H + c.c.) .
  \end{equation}

  \item A complex $SU(2)_L$ quartet scalar $\Phi_{3/2}$ ($\Phi_{1/2}$) with hypercharge $Y_\Phi=\frac{3}{2}$ ($Y_\Phi=\frac{1}{2}$)
  \begin{equation}
  \Delta \mathcal{L} \supset \Phi^\dag H^3 + c.c. ,
  \end{equation}

%  \item A heavy $U(1)$ gauge boson $K_\mu$
%  \begin{equation}
%  \Delta \mathcal{L} \supset B^{\mu\nu} K_{\mu\nu} ,
%  \end{equation}
%  where $K_{\mu\nu}=\partial_\mu K_\nu-\partial_\nu K_\mu$ and $B_\mu$ denotes the SM $U(1)_Y$ gauge boson.
\end{enumerate}

%We now show that the above list exhausts the possibilities of tree-level Wilson coefficients from renormalizable UV models in which heavy states only couple with the bosonic fields of the SM. In order to have tree-level generated Wilson coefficients, the UV Lagrangian must contain a term that is linear in the heavy field. We therefore need not consider heavy fermion fields \(\Psi\) since Lorentz invariance requires that a linear term in \(\Psi\) couples to some SM fermion. A heavy vector boson has to be gauged in order for the UV theory to be renormalizable. By our requirement of only coupling to SM bosons, SM fermions must be singlets under this gauge symmetry; the non-zero yukawa couplings (together with renormalizabilty) then tell us the Higgs is also singlet under this gauge symmetry. Thus, the massive gauge boson can only couple to SM gauge bosons and one easily sees that No.5 above is the only possibility.

%The only case left is a heavy scalar $\Phi$ that couples to the SM Higgs $H$ and gauge bosons. A renormalizable interaction term between $\Phi$ and the SM gauge bosons cannot be linear in $\Phi$ due to gauge invariance. Therefore, what is left for us is to count all the possible Lagrangian terms formed by $\Phi$ and $H$ that are linear in $\Phi$. After appropriate diagonalization of $\Phi$ and $H$, we do not need to consider the quadratic terms. Then there are only two types of renormalizable interactions $H^aH^b\Phi^{ab}$ and $H^aH^bH^c\Phi^{abc}$, where we have written the SM Higgs field $H$ in terms of its four real components $H^a$ with $a=1,2,3,4$. Because only symmetric combinations are non-vanishing, it is clear that there are in total $10$ real components $\Phi^{ab}$ that are enumerated by No.1 and No.2 in the above list, and $20$ real components $\Phi^{abc}$ that are enumerated by No.3 and No.4.

We now show that the above list exhausts the possibilities of heavy scalars that couple via renormalizable interactions to the Higgs and produce tree-level Wilson coefficients. In order to have tree-level generated Wilson coefficients, the UV Lagrangian must contain a term that is linear in the heavy field. Therefore, we need to count all possible Lagrangian terms formed by $\Phi$ and $H$ that are linear in $\Phi$. After appropriate diagonalization of $\Phi$ and $H$, we do not need to consider the quadratic terms. Then there are only two types of renormalizable interactions $H^aH^b\Phi^{ab}$ and $H^aH^bH^c\Phi^{abc}$, where we have written the SM Higgs field $H$ in terms of its four real components $H^a$ with $a=1,2,3,4$. Because only symmetric combinations are non-vanishing, it is clear that there are in total $10$ real components $\Phi^{ab}$ that are enumerated by No.1 and No.2 in the above list, and $20$ real components $\Phi^{abc}$ that are enumerated by No.3 and No.4.

In the rest of this subsection, we will discuss in detail the examples above and compute their effective actions through one-loop order. Additionally, we will also compute the one-loop effective action of three other examples: (1) degenerate scalar tops in the MSSM, (2) a heavy \(U(1)\) gauge boson that kinetically mixes with hypercharge, and (3) massive \(SU(2)\) vector bosons that couple universally to fermions. The latter model can arise in extra-dimension and little Higgs theories.

\textcolor{blue}{When there is a non-zero tree-level contribution, \(\Ph_c \ne 0\), the dependence of the one-loop functional determinant on the classical configuration can introduce divergences into the Wilson coefficients of operators with dimension greater than four. These terms generically are associated with renormalization of parameters in the UV Lagrangian (see the discussion at the beginning of Sec.~\ref{sec:CDE_summary}, around Fig.~\ref{fig:CDEdiagrams}). Therefore, the effects of the contributions can be absorbed into a redefinition (renormalization scheme dependence) of the UV Lagrangian parameters, and hence dropped from the matching analysis. Another natural scheme choice is to use \(\xoverline{\text{MS}}\). In \(\xoverline{\text{MS}}\) scheme, from Eq.~\eqref{eqn:CDE_universal_lag}, there is a finite contribution to higher dimension operators from the \(\tr\, U\) piece. To show where this difference arises in doing calculations, in our examples of the triplet scalar and doublet scalar we will use the \(\xoverline{\text{MS}}\) renormalization scheme, while for all the other examples we will absorb the divergences of HDOs into the UV Lagrangian parameters. For the latter case, this essentially amounts to dropping \(\Ph_c\) from the one-loop calculation.} %One can always redefine the parameters of the UV Lagrangian in some renormalization scheme so that this where these 

%In the matching process, such divergences are associated with terms proportional to \(\log (m^2/\m^2)\) in Eq.~\eqref{eqn:CDE_universal_lag}, namely when \(\tr \, U\) or \(\tr \, U^2\) contain higher dimension operators. In the examples considered, we present the Wilson coefficients at the matching scale \(\m = m\) and adopt the \(\xoverline{\text{MS}}\) regularization scheme, as in Eq.~\eqref{eqn:CDE_universal_lag}. In this scheme, there is a non-zero finite piece associated to \(\tr \, U\), while it vanishes for the \(\tr \, U^2\) term.}

%In totatility, the seven examples we consider include different types of species and come at varying levels of complexity. This serves two purposes. In the arena of pedagogy, we hope to show how details are handled for actual computations a reader might be interested in performing. In the arena of demonstrating the utility of the CDE, the more complicated the example, the more the CDE saves over traditional methods.

\renewcommand\arraystretch{1.4}
\begin{table}[tb]
\centering
\begin{tabular}{|rcl|rcl|}\hline
 \(\scO_{GG}\) &\(=\)& \(g_s^2 \abs{H}^2G_{\mu \nu }^aG^{a,\mu \nu }\) & \(\scO_H\)   &\(=\)& \(\frac{1}{2}\big(\pd_{\mu} \abs{H}^2\big)^2\)\\
%
 \(\scO_{WW}\) &\(=\)& \(g^2  \abs{H}^2 W_{\mu \nu }^aW^{a,\mu \nu } \) &  \(\scO_T\)   &\(=\)& \(\frac{1}{2}\big( H^{\dag} \Dfbd H\big)^2\) \\
%
 \(\scO_{BB}\) &\(=\)& \(g'^2 \abs{H}^2 B_{\mu \nu }B^{\mu \nu }\) & \(\scO_R\)   &\(=\)& \(\abs{H}^2\abs{D_{\m}H}^2\) \\
%
 \(\scO_{WB}\) &\(=\)& \(2gg'H^\dag {\tau^a}H W_{\mu \nu }^a B^{\mu \nu }\) &  \(\scO_D\)   &\(=\)& \(\abs{D^2H}^2\) \\
%
 \(\scO_W\)   &\(=\)& \(ig\big(H^\dag \tau^a \Dfb H\big)D^\nu W_{\mu \nu }^a\) &  \(\scO_6\)   &\(=\)& \(\abs{H}^6\) \\
%
 \(\scO_B\)   &\(=\)& \(ig'Y_H\big(H^\dag \Dfb H\big)\pd^\nu B_{\mu \nu }\)  &  \(\scO_{2G}\) &\(=\)& \(-\frac{1}{2} \big(D^\mu G_{\mu \nu }^a\big)^2\) \\
%
 \(\scO_{3G}\) &\(=\)& \(\frac{1}{3!}g_sf^{abc}G_\rho ^{a\mu }G_\mu ^{b\nu }G_\nu ^{c\rho }\) &  \(\scO_{2W}\) &\(=\)& \(-\frac{1}{2} \big(D^\mu W_{\mu \nu }^a\big)^2\) \\
%
 \(\scO_{3W}\) &\(=\)& \(\frac{1}{3!}g \e^{abc}W_\rho ^{a\mu }W_\mu ^{b\nu }W_\nu ^{c\rho }\) & \(\scO_{2B}\) &\(=\)& \(-\frac{1}{2} \big(\pd^{\mu} B_{\mu \nu }\big)^2\) \\
  \hline
\end{tabular}
\caption{CP conserving dimension-six bosonic operators.} \label{tbl:operators}
\vspace{-10pt}
\end{table}
\renewcommand\arraystretch{0}

\subsubsection{Electroweak triplet scalar}

Let us consider an electroweak triplet scalar \(\Ph\) with neutral hypercharge. The Lagrangian contains the trilinear interaction \(H^{\dag}\Ph H\), where \(H\) is the electroweak Higgs doublet. This interaction, being linear in \(\Ph\), leads to a tree-level contribution to the effective action when we integrate out \(\Ph\).

While our main purpose here is to demonstrate how to use the CDE, we note that EW triplet scalars are phenomenologically interesting~\cite{Georgi:1985nv,*Chanowitz:1985ug} and well studied (for a recent study of triplet collider phenomenology and constraints see, \textit{e.g.},~\cite{Englert:2013wga}). As shown below, the electroweak \(T\) parameter is generated at tree-level due to the custodial violating interaction \(H^{\dag}\Ph H\). The strong constraints on the \(T\) parameter require the triplet scalar to have a large mass, \(m \gg v\). In this regime, the leading terms of the EFT are quite accurate.

For readers interested in comparing the CDE with traditional Feynman diagram techniques, we note that triplet scalars were studied within the EFT framework in~\cite{Khandker:2012,*Skiba:2010} where the Wilson coefficients were calculated using Feynman diagrams (see the appendices of~\cite{Khandker:2012,*Skiba:2010}). Tree-level Feynman diagrams involving scalar propagators are straightforward to deal with; yet, we believe that even in this simple case the CDE offers a significantly easier method of calculation. In particular, at no point do we (1) have to break the Lagrangian into gauge non-covariant pieces to obtain Feynman rules, (2) look up a table of higher dimension operators to know how to rearrange the answer back into a gauge-invariant form, or (3) consider various momenta configurations of external particles in order to extract which particular higher dimension operator is generated.

\begin{center} \small{\textbf{Tree-level matching}} \end{center}

Let \(\Ph = \Ph^aT^a\) be an electroweak, real scalar triplet with hypercharge \(Y_{\Ph}=0\).\footnote{For \(Y_{\Ph} \ne 0\), \(\Ph^a\) must be complex. Only for \(Y_{\Ph} = 0 \text{ or }1\) can \(\Ph\) have a trilinear interaction with \(H\).} We take the \(SU(2)_L\) generators in the fundamental representation, \(T^a = \t^a = \s^a/2\) with \(\s^a\) the Pauli matrices. The Lagrangian involving \(\Ph\) and its interactions with the Standard Model Higgs doublet is given by\footnote{The coupling names and normalization are chosen to coincide with those in~\cite{Khandker:2012,*Skiba:2010}.}
\begin{equation}
\scL[\Ph,H] = \frac{1}{2} \big( D_{\m}\Ph^a\big)^2 - \frac{1}{2} m^2\Ph^a\Ph^a +2\k H^{\dag}\t^a H \Ph^a - \et \abs{H}^2\Ph^a\Ph^a -\frac{1}{4}\l_{\Ph}(\Ph^a\Ph^a)^2,
\label{eqn:lag_triplet}
\end{equation}
where \(D_{\m}\Ph = [D_{\m},\Ph] = (\pd_{\m}\Ph^a + g\e^{abc}W_{\m}^b\Ph^c)T^a = (D_{\m}\Ph^a)T^a\). The interaction \(H^{\dag}\Ph H\), being linear in \(\Ph\), leads to a tree-level contribution to the effective action. To calculate this contribution, we follow the steps outlined in section~\ref{sec:CDE_tree}. Introducing an obvious vector notation and writing the Lagrangian as in Eq.~\eqref{eqn:tree_UV_Lag},
\begin{equation}
\scL = \frac{1}{2} \vec{\Ph}^T \big(P^2 - m^2 - U\big) \vec{\Ph} + \vec{\Ph}\cdot\vec{B} + \scO(\Ph^3), \quad U = 2 \et \abs{H}^2 \text{ and } \vec{B} = 2\k H^{\dag}\vec{\t} H,
\label{eqn:lag_triplet2}
\end{equation}
we solve the equation of motion for \(\Ph\) and plug it back into the action. Linearizing the equation of motion,\footnote{At tree-level, the quartic \((\vec{\Ph}\cdot\vec{\Ph})^2\) term contributes only to dimension eight and larger operators, and we therefore ignore it presently. The quartic piece does lead to a contribution of the one-loop effective action, which is discussed below.} we have
\begin{equation}
\vec{\Ph}_c = -\frac{1}{P^2 - m^2 - U} \vec{B}.
\label{eqn:trip_Ph_c}
\end{equation}
The tree-level effective action is given by \(\scL_{\text{eff,tree}}[H] = \scL[\Ph_c,H]\). Performing an inverse mass expansion on \(\Ph_c\), the effective action through dimension-six operators is, %given as in Eq.~\eqref{eqn:tree_cde_terms},
\[
\scL_{\text{eff,tree}} = \frac{1}{2m^2}\vec{B}\cdot\vec{B} +\frac{1}{2m^4}\vec{B}^T\big(P^2 - U\big)\vec{B} + \text{ dim 8 operators},
\]
\textcolor{blue}{where the factor of two difference from Eq.~\eqref{eqn:tree_cde_terms} occurs because \(\vec{\Ph}\) is real.}

Now we need to evaluate the terms in the above. For the \(\vec{B}\cdot \vec{B}\) term we have\footnote{Here and below we use the following relation for generators \(T^a\) in the fundamental representation of \(SU(N)\): \((T^a)_{ij}(T^a)_{kl} = \frac{1}{2}(\d_{il}\d_{jk} - \frac{1}{N}\d_{ij}\d_{kl})\).}
\begin{equation*}
B^aB^a = 4\k^2(H^{\dag}\t^aH)(H^{\dag}\t^aH) = \k^2 \abs{H}^4,
\end{equation*}
from which it follows
\begin{equation*}
B^aUB^a = 2\et \k^2 \abs{H}^6.
\end{equation*}
Integrating by parts, the term in involving the covariant derivative is \(\vec{B}^{T} (-D^2) \vec{B} = (D_{\m}\vec{B})^2\) where
\begin{equation*}
D_{\m}B^a \propto D_{\m}(H^{\dag}\t^aH) = (D_{\m}H)^{\dag}\t^aH+ H^{\dag}\t^a(D_{\m}H) .
\end{equation*}
Squaring this, using the identity in the previous footnote and the one in Eq.~\eqref{eqn:cdeA_opsq} we have
\begin{align*}
(D_{\m}B^a)^2 &= \k^2 \big(H^{\dag}\Dfb H \big)^2 + 4\k^2 \abs{H}^2\abs{D_{\m}H}^2 \\
&= 2\k^2 \big(\scO_T + 2\scO_R \big) ,
\end{align*}
where \(H^{\dag}\Dfb H = H^{\dag}(D_{\m}H) - (D_{\m}H)^{\dag}H\) and the operators \(\scO_{T,R}\) are as defined in Table~\ref{tbl:operators}.

Putting it all together, we find
\begin{equation}
\scL_{\text{eff,tree}} = \frac{\k^2}{2m^2} \abs{H}^4 + \frac{\k^2}{m^4} \big(\scO_T + 2\scO_R \big) - \frac{\et \k^2}{m^4} \scO_6 ,
\label{eqn:triplet_tree}
\end{equation}
where \(\scO_6 = \abs{H}^6\). As mentioned previously, these results were also obtained in~\cite{Khandker:2012,*Skiba:2010} using Feynman diagrams.\footnote{The notation in the first reference of~\cite{Khandker:2012,*Skiba:2010} uses the three operators \(\scO_1\), \(\scO_2\), and \(\scO_T'\) where we added the prime since it is not the same as our \(\scO_T\). What they call \(\scO_T'\) is now more commonly called \(\scO_{HD}\). In our notation, \(\scO_T' = \abs{H^{\dag}D_{\m}H}^2 \equiv \scO_{HD} = (\scO_H - \scO_T)/2\), \(\scO_1 = -(\scO_R + \scO_H)\), and \(\scO_2 = \scO_R\).} The first term in the above can be absorbed into the renormalization of the Higgs quartic coupling. As we will discuss in section~\ref{sec:mapping}, \(\scO_T\) contributes to the electroweak \(T\) parameter. Thus, we see in the effective theory that the \(T\) parameter is generated at tree-level.

\begin{center} \small{\textbf{One-loop level matching}} \end{center}


\begin{figure}[t]
\centering
 \subfigure{
 \centering
\begin{fmffile}{H4}
\begin{fmfgraph*}(50,20)
\fmfleft{i1,i2}
\fmfright{o1,o2}
\fmftop{t}
\fmfbottom{b}
\fmflabel{$H^\dagger$}{i2}
\fmflabel{$H$}{i1}
\fmflabel{$H^\dagger$}{o2}
\fmflabel{$H$}{o1}
\fmf{scalar}{i1,i,i2}
\fmf{scalar}{o1,o,o2}
\fmf{phantom,tension=1.2}{p,b}
\fmf{plain,tension=2}{i,p,o}
\fmf{plain,left,tension=0.6}{p,t,p}
\end{fmfgraph*}
\end{fmffile}
 }\hspace{2cm}
 \subfigure{
 \centering
\begin{fmffile}{H6}
\begin{fmfgraph*}(50,35)
\fmfleft{i1,i2,i3}
\fmfright{o1,o2,o3}
\fmfbottom{b}
\fmflabel{$H^\dagger$}{i2}
\fmflabel{$H$}{i1}
\fmflabel{$H^\dagger$}{o2}
\fmflabel{$H$}{o1}
\fmflabel{$H^\dagger$}{o4}
\fmflabel{$H$}{i4}
\fmf{phantom,tension=1.0}{i3,i4}
\fmf{phantom,tension=1.0}{o3,o4}
\fmf{phantom,tension=2}{p,b}
\fmf{scalar}{i1,i,i2}
\fmf{scalar}{o1,o,o2}
\fmf{scalar}{i4,v,o4}
\fmf{plain,tension=2.5}{i,p,o}
\fmf{plain,left,tension=1.0}{p,v,p}
\end{fmfgraph*}
\end{fmffile}
 }
 \caption{Feynman diagrams for $\vec{\Ph}_c \ne 0$ effects at one-loop.%, which can be clearly absorbed into the renormalization of $m^2$.
} \label{fig:RGtermdiagrams}
\end{figure}


Let us also calculate the one-loop effective action from integrating out the scalar triplet. It is given by
\begin{equation*}
\D S_{\text{eff,1-loop}} = \frac{i}{2} \Tr \log \left[ - \left. \frac{\d^2S}{\d \Ph^2} \right|_{\Ph = \Ph_c} \right] = \frac{i}{2} \Tr \log \big[ -P^2 + m^2 + U' \big],
\end{equation*}
with
\begin{equation*}
U' = 2\et \abs{H}^2 \cdot \mathbf{1}_3+ \l_{\Ph} \Big[\big(\vec{\Ph}^T_c\cdot \vec{\Ph}_c\big)  \cdot \mathbf{1}_3 + 2 \vec{\Ph}_c \vec{\Ph}_c^T\Big],
\end{equation*}
where \(\mathbf{1}_3\) is the \(3\times 3\) identity matrix and we explicitly wrote it above to remind the reader that each piece in \(U'\) is a matrix. The term in square brackets above is due to the fact that there is a non-zero tree-level piece, \textit{i.e.} that \(\vec{\Ph}_c \ne 0\). \textcolor{blue}{Diagrammatically, this term leads to connected, but not 1PI, diagrams of the sort shown in Fig.~\ref{fig:RGtermdiagrams}. Such diagrams are clearly associated with renormalization of parameters in the UV Lagrangian, \textit{e.g.} \(\Ph\)'s mass \(m\) in Fig.~\ref{fig:RGtermdiagrams}. We recall that \(\Ph_c\) is given by Eq.~\eqref{eqn:trip_Ph_c},} %(see also the discussion at the beginning of Sec.~\ref{sec:CDE_summary}, around Fig.~\ref{fig:CDEdiagrams}).
\[
\vec{\Ph}_c = \frac{1}{m^2}\vec{B} + \frac{1}{m^4}(P^2 - U)\vec{B} + \dots.
\]

%To leading order, we can take the lowest order solution of \(\Ph_c\) in Eq.~\eqref{eqn:trip_Ph_c}, namely
%\[
%\vec{\Ph}_c \approx \frac{1}{m^2}\vec{B} = \frac{2\k}{m^2} H^{\dag}\vec{\t}H.
%\]
%With this, \(U'\) is given by
%\[
%U' = U + \frac{\l_{\Ph}}{m^4} \Big[ \vec{B}^T \vec{B} + 2\vec{B}\vec{B}^T\Big] = U +  \frac{\l_{\Ph} \k^2}{m^4} \Big[ \abs{H}^4 + 8 \big(H^{\dag}\vec{\t}H\big)\big(H^{\dag}\vec{\t}H\big)^T \Big],
%\]
%where \(U = 2\et\abs{H}^2\)  as in Eq.~\eqref{eqn:lag_triplet2}.

To evaluate the one-loop effective action, we take the universal results from Eq.~\eqref{eqn:CDE_universal_lag} with \(c_s = 1/2\) since \(\Ph^a\) is a real scalar. As \(U'\) contains no term that is linear in fields, for dimension six and less operators we take the \(m^2\), \(m^0\), and \(m^{-2}\) terms from Eq.~\eqref{eqn:CDE_universal_lag}
\begin{align}
32\pi^2&\D \scL_{\text{eff,1-loop}} = -m^2\Big(\log \frac{m^2}{\m^2} - 1\Big) \tr \, U' -\frac{1}{12}\Big(\log \frac{m^2}{\m^2} - 1\Big) \tr \, G_{\m\n}'^2 - \frac{1}{2} \log \frac{m^2}{\m^2} \tr \, U'^2 \nonumber \\
& +\frac{1}{m^2} \bigg[- \frac{1}{60} \tr \big(P_{\m}G_{\m\n}'\big)^2 - \frac{1}{90} \tr \, G_{\m\n}'G_{\n\s}'G_{\s\m}' -\frac{1}{12}\tr \, (P_{\m}U')^2 - \frac{1}{6}\tr \, U'^3 - \frac{1}{12} \tr \, U' G_{\m\n}'G_{\m\n}' \bigg].
\label{eqn:trip_oneloop_gen}
\end{align}
We are interested in the dimension-six operators generated by integrating out \(\Ph\); since the \(\scO(\Phi_c^2)\) term in \(U'\) is minimally quartic in SM fields, \(\scO(\Ph_c^2) \sim \scO(H^4)+\dots\), we can set \(U' \approx U = 2\et\abs{H}^2\) in the second line of the above equation. In the first line of~\eqref{eqn:trip_oneloop_gen}, higher dimension operators arise because \(\Ph_c \ne 0\); by simple power counting, to capture the dim-6 operators we need to take \(\Ph_c \approx \vec{B}/m^2 + (P^2 - U) \vec{B}/m^4\) in the \(\tr \, U'\) term and \(\Ph_c \approx \vec{B}/m^2\) in the \(\tr \, U'^2\) term.%Besides an \(\abs{H}^6\) term in \(\tr \, U'^2\), the first line in~\eqref{eqn:trip_oneloop_gen} does not contain dimension-six operators.
\footnote{As a side comment, we note that the terms in the first line of Eq.~\eqref{eqn:trip_oneloop_gen} can be used to find the contribution of \(\Ph\) to the beta functions of SM couplings. In particular, the triplet contributes to the running of the Higgs' mass and quartic coupling and also to the \(SU(2)_L\) gauge coupling \(g\). This is easy to see since
\begin{align*}
\tr \, U' &= 3 U + 5 \frac{\l_{\Ph}}{m^4} \vec{B}^T\vec{B} + \text{ dim-six ops } = 6\et \abs{H}^2 + 5\frac{\l_{\Ph}\k^2}{m^4}\abs{H}^4 \\
\tr \, U'^2 &= 3 U^2 + \text{ dim-six ops } = 12 \et^2 \abs{H}^4 + \dots \\
\tr G_{\m\n}'^2 &= -2 g^2 (W_{\m\n}^a)^2.
\end{align*}
} %The second line in the above contains the dimension six operators generated at one loop.

To evaluate the traces in~\eqref{eqn:trip_oneloop_gen}, recall that \(G_{\m\n}' = [D_{\m},D_{\n}]\). Since \(\Ph\) is in the adjoint of \(SU(2)_L\), \(G_{\m\n}' = [D_{\m},D_{\n}] = -ig W_{\m\n}^at^a_G\) where the generators \(t^a_G\) are in the adjoint representation, so \(\tr(t^a_Gt^b_G) = 2 \d^{ab}\). %\footnote{For \(SU(N)\), \(\tr(t^a_Gt^b_G) = N \d^{ab}\).}
Keeping only up to dimension-six operators and using the operator definitions given in table~\ref{tbl:operators}, the traces evaluate to\footnote{For example,
\begin{align*}
\tr \, U'^2 &= \tr \, \Big[U \cdot \mathbf{1}_3 + \frac{\l_{\Ph}}{m^4}\Big(\vec{B}^T\vec{B} \cdot 1_{3 \times 3} + 2 \vec{B}\vec{B}^T\Big) \Big]^2 \\
&\supset 2 \frac{\l_{\Ph}}{m^4}\, U\cdot  \tr \, \Big(\vec{B}^T\vec{B} \cdot 1_{3 \times 3} + 2 \vec{B}\vec{B}^T\Big) \\
&= 2 \frac{\l_{\Ph}}{m^4}\, U \cdot \big(5 \vec{B}^T\vec{B} \big) \Rightarrow U = 2\et \abs{H}^2, \ \vec{B}^T\vec{B} = \k^2 \abs{H}^4 \Rightarrow\\
&= 20 \, \frac{\k^2 \et \l_{\Ph} }{m^4} \, \abs{H}^6
\end{align*}
}
\[
\def\arraystretch{1.4}
\begin{array}{rclll}
\tr \, U' & \supset & 5 \l_{\Ph}\vec{\Ph}_c^2 & \supset & 20 \dfrac{\l_{\Ph} \k^2}{m^6}\big(-\et \scO_6 + \scO_T + 2\scO_R\big) \\
\tr \, U'^2 & \supset & 20 \, \dfrac{\l_{\Ph} \k^2 \et }{m^4} \, \abs{H}^6 & = & 20 \, \dfrac{\k^2 \et \l_{\Ph} }{m^4} \scO_6\\
\tr \, U^3 &=& 3 \big(2\et \abs{H})^3 & = & +24\et^3 \scO_6 \\
\tr \big(P_{\m}U\big)^2 & = & -3 \big(2\et \pd_{\m} \abs{H}^2\big)^2 &=& -24 \et^2 \scO_H \\
\tr UG_{\m\n}'G_{\m\n}' & = & -4\et g^2 \abs{H}^2 \big(W_{\m\n}^a\big)^2 &=& -4\et \scO_{WW}\\
 \tr G'^3 & = & -g^3 \e_{abc}W_{\m\n}^aW_{\n\s}^bW_{\s\m}^c& = & -6g^2 \scO_{3W} \\
\tr \big(P_{\m}G_{\m\n}'\big)^2 & = & 2g^2 \big(D_{\m}W_{\m\n}^a)^2 &=& -4 g^2 \scO_{2W}
\end{array}
\]
Plugging these back into~\eqref{eqn:trip_oneloop_gen}, the dimension-six operators in the one-loop effective action are
%\begin{equation}
%\D \scL_{\text{eff,1-loop,dim 6}} = \frac{1}{32\pi^2} \frac{1}{m^2} \bigg[ \frac{g^2}{15}\Big(\scO_{2W} + \scO_{3W}\Big) + 2 \et^2 \,\scO_H + \frac{\et}{3} \scO_{WW} - 4\et^3 \scO_6  \bigg].
%\end{equation}
\begin{align}
\D \scL_{\text{eff,1-loop,dim 6}} = \frac{1}{32\pi^2} \frac{1}{m^2} \bigg[ \frac{g^2}{15}\Big(\scO_{2W} + \scO_{3W}\Big) &+ 2 \et^2 \,\scO_H + \frac{\et}{3} \scO_{WW} - 4\et^3 \scO_6 \nonumber \\
&+ 20 \frac{\l_{\Ph}\k^2}{m^2} \Big(-\et \scO_6 + \scO_T + 2\scO_R\Big) \bigg].
\end{align}
\textcolor{blue}{Note that for the present example we use \(\xoverline{\text{MS}}\) renormalization scheme, whose scheme-dependent finite pieces manifest as the terms proportional to \(\l_{\Ph}\) in the above. These terms are associated to the renormalization of the \(\Ph\) mass and the coupling cross-quartic coupling \(\et\), see Fig.~\ref{fig:RGtermdiagrams}; one can in principle choose a different scheme so that these contributions vanish. Finally, we reiterate that the above effective Lagrangian is at the matching scale \(\m = m\), hence why the logarithm pieces from Eq.~\eqref{eqn:trip_oneloop_gen} vanish (this is scheme-independent).}
%\textcolor{blue}{Note that this is at the matching scale \(\m = m\), hence why the contribution to \(\scO_6\) from the \( \tr\, U'^2\) term in \eqref{eqn:trip_oneloop_gen} vanishes.}

\subsubsection{Extra EW scalar doublet}
Here we integrate out an additional electroweak scalar doublet \(\Ph\) with hypercharge \(Y_\Ph = -1/2\) and mass \(m^2 \gg v^2\). This is essentially the two Higgs doublet model (2HDM) where the mass term for the extra scalar is taken large compared to the EW symmetry breaking scale.

The general Lagrangian for a 2HDM model can be rather complex; often, if the UV model doesn't already impose some restriction on the 2HDM model (as it does in, \textit{e.g.}, supersymmetry), then some other simplifying approximation is made to make more tractable the study of the second doublet. Below, we will consider the most general scalar sector for the second EW doublet; this is rather easy to handle within our EFT framework and requires little additional effort.\footnote{Of course, a large reason why this is much easier in the EFT framework is because we have made the simplifying assumption that the second doublet is heavy.}

The most general Lagrangian consisting of an extra EW scalar doublet \(\Ph\) with \(Y_{\Ph} = -1/2\) interacting with the Higgs sector is given by
\begin{align}
\scL \supset &\abs{D_{\m}\Ph}^2 - m^2 \abs{\Ph}^2 - \frac{\l_{\Ph}}{4}\abs{\Ph}^4 \nonumber\\
&+ \big(\et_H \abs{\tH}^2+\et_{\ph}\abs{\Ph}^2\big)\big(\tH^{\dag}\Ph + \Ph^{\dag}\tH\big) \nonumber\\
&-\l_1\abs{\tH}^2\abs{\Ph}^2 - \l_2 \abs{\tH^{\dag}\Ph}^2 -\l_3 \big[\big(\tH^{\dag}\Ph\big)^2 + \big(\Ph^{\dag}\tH\big)^2 \big].
\label{eqn:EW_doub_lag}
\end{align}
where \(D_{\m}\Ph = (\pd_{\m} - i g W_{\m}^a \t^a - ig' Y_{\Ph} B_{\m})\Ph\), \(\t^a = \s^a/2\) are the \(SU(2)_L\) generators in the fundamental representation, and \(\tH \equiv i \s_2 H^*\) \textcolor{blue}{so that \(\e^{\a\b}\Ph_{\a}H_{\b} = \tH^{\dag}\Ph\)}. The first line of the above is the potential of \(\Ph\) alone, the second line contains a linear term in \(\Ph\) which leads to a tree-level contribution to the effective action, while the last line contains interactions with the Higgs doublet \(H\) that appear in the effective action at one-loop order.

The main purpose of this section is to show how to use the covariant derivative expansion; in this regard, we remain agnostic to restrictions specific 2HDM models might impose on the Lagrangian in~\eqref{eqn:EW_doub_lag}. However, let us make a few, brief comments. Here we focus on the Higgs sector and have not included a Yukawa sector with couplings to \(\Ph\); these would lead to tree-level generated dimension-six operators involving only fermions. If a parity \(\Ph \to -\Ph, H \to H\) is imposed, then the terms in the second line of~\eqref{eqn:EW_doub_lag} and extra Yukawa terms are forbidden. This parity prevents \(\Ph\) from developing a vacuum expectation value\footnote{Since we assume \(m^2 >0\), \(\Ph\) can only get a vacuum expectation value via the term linear in \(\Ph\) in~\eqref{eqn:EW_doub_lag}, \textit{i.e.} the \(\et_{\Ph}\abs{H}^2\big(\tH^{\dag} \Ph + \text{h.c.}\big)\) term.} and \(\Ph\) in this case is sometimes known as an ``inert Higgs''~\cite{Barbieri:2006}. Finally, imposing an exact or approximate global \(U(1)\) on \(\Ph\) eliminates the second line in~\eqref{eqn:EW_doub_lag}, the term proportional to \(\l_3\) in~\eqref{eqn:EW_doub_lag}, and any potential Yukawa terms involving \(\Ph\).

\begin{center} \small{\textbf{Tree-level matching}} \end{center}

When we integrate out the massive doublet the term linear in \(\Ph\) in~\eqref{eqn:EW_doub_lag}, \(\et_{H}\abs{H}^2\big(\tH^{\dag} \Ph + \text{h.c.}\big)\), leads to a tree-level contribution to the effective action. As this interaction is cubic in the Higgs field, it is simple to see that the only dimension-six operator will be \(\scO_6 = \abs{H}^6\). Concretely, \(B\) from the general tree-level formula Eq.~\eqref{eqn:tree_cde_terms} is given by \(B = \et_{H} \abs{H}^2 \tH\). The solution to the linearized equation of motion is
\begin{equation}
\Ph_c = -\frac{1}{P^2 - m^2 - \l_1 \abs{H}^2 - \l_2 \tH\tH^{\dag}}B \approx \frac{1}{m^2}B = \frac{\et_H}{m^2}\abs{H}^2 \tH ,
\label{eqn:doub_Ph_c}
\end{equation}
and the tree-level effective action through dimension-six operators is
\begin{equation}
\D \scL_{\text{eff,tree,dim-6}} = \frac{1}{m^2} B^{\dag}B = \frac{\et_{H}^2}{m^2} \abs{H}^6 =  \frac{\et_{H}^2}{m^2} \scO_6 .
\label{eqn:EW_doub_tree}
\end{equation}

\begin{center} \small{\textbf{One-loop-level matching}} \end{center}

Let us now find the one-loop effective action from integrating out the massive scalar doublet \(\Ph\) in Eq.~\eqref{eqn:EW_doub_lag}. One of the main reasons we provide these examples is to show how to use the covariant derivative expansion. All the couplings in Eq.~\eqref{eqn:EW_doub_lag} make the effective action calculation complicated, but not very difficult. For the moment, however, let us make several simplifying assumptions on the couplings simply so that the basic setup and use of the CDE is not obscured. After we show the CDE for the simpler Lagrangian, we will return to the full Lagrangian in Eq.~\eqref{eqn:EW_doub_lag} and use the CDE to compute the one-loop effective action.\\

\noindent \textit{Simplifying case}\\

For the simplifying assumptions, let us impose a global \(U(1)\) on \(\Ph\) so that \(\et_H = \et_{\Ph} = \l_3 = 0\) in the Lagrangian. Again, we will come back and let these terms be non-zero shorty. In this case, there is no tree-level effective action. We integrate \(\Ph\) out of the Lagrangian
\[
\scL \supset \Ph^{\dag}\big( -D^2 -m^2 - \l_1 \abs{H}^2 - \l_2 \tH \tH^{\dag} \big) \Ph.
\]
After performing the gaussian integral we are left with the effective action
\[
\D S_{\text{eff,1-loop}} = i\text{Tr}\log\big[ -P^2 + m^2 + A \big],
\]
where we defined
\begin{equation}
A \equiv \l_1 \abs{H}^2 + \l_2 \tH \tH^{\dag}.
\label{eqn:doub_A_def}
\end{equation}
From here, we can use the univeral formula in Eq.~\eqref{eqn:CDE_universal_lag} with \(c_s = 1\) since \(\Ph\) is a complex boson and \(A\) substituted for \(U\) in~\eqref{eqn:CDE_universal_lag}. At this point, we are essentially done; all that is left is to compute the traces.

Let us give a few examples of trace computations by considering \(\tr \big( G_{\m\n}' G_{\n\s}'G_{\s\m}'\big)\) and \(\tr \big( A G_{\m\n}'G_{\m\n}'\big)\). The covariant derivative acting on \(\Ph\) is \(D_{\m} = \pd_{\m} - i g W_{\m} - i g' Y_{\Ph} B_{\m}\cdot \mathbf{1}_2\) where we have explicitly denoted the \(2\times 2\) identity matrix by \(\mathbf{1}_2\). Therefore,
\[
G_{\m\n}' = [D_{\m},D_{\n}] = - ig W_{\m\n}^a \t^a - ig' Y_{\Ph}B_{\m\n} \cdot \mathbf{1}_2.
\]
In \(\tr G'^3\) the anti-symmetry on the Lorentz indices only leaves \(\tr W^3\) non-vanishing. Thus,\footnote{We used
\[
\tr \big(T^a T^b T^c\big) = \frac{1}{2} \tr \Big( [T^a,T^b]T^c + \underbrace{\{T^a,T^b\}T^c}_{\text{vanishes by }W^aW^bW^c\text{ anti-symm}} \Big) = \frac{i}{2}f^{abd}\tr T^dT^c = \frac{i}{2} \m(R) f^{abc}
\]
}
\[
\tr \, G_{\m\n}' G_{\n\s}'G_{\s\m}' = i g^3 \tr \, W_{\m\n}W_{\n\s}W_{\s\m} = -\frac{g^3}{2} \m(R) \e_{abc} W_{\m\n}^aW_{\n\s}^bW_{\s\m}^c = -3g^2 \m(R) \scO_{3W} ,
\]
where \(\m(R)\) is the Dynkin index for representation \(R\) and is equal to \(1/2\) for the fundamental representation and \(\scO_{3W}\) is as defined in table~\ref{tbl:operators}.

For \(\tr \big( A G_{\m\n}'G_{\m\n}'\big)\) we have
\begin{align*}
\tr \big( A G_{\m\n}'G_{\m\n}'\big) &= - \tr\Big[ A \times \big(g W_{\m\n}^a\t^a +g'Y_{\Ph}B_{\m\n} \cdot \mathbf{1}_2)^2 \Big]\\
&=  -g^2 \tr \big(A W_{\m\n}W_{\m\n} \big) - g'^2Y_{\Ph}^2B_{\m\n}B_{\m\n}\tr\, A - 2gg'Y_{\Ph}B_{\m\n}\tr\big(A W_{\m\n}\big) ,
\end{align*}
using \(\tr A \t^a = \l_2 \tH^{\dag}\t^a \tH = -\l_2 H^{\dag}\t^a H\) and a few other manipulations, it is straightforward to see that
\begin{align*}
\tr \big( A G_{\m\n}'G_{\m\n}'\big) &= - (2\l_1 + \l_2)\Big(\frac{g^2}{4} \abs{H}^2 W_{\m\n}^aW_{\m\n}^a   +g'^2 Y_{\Ph}^2\abs{H}^2 B_{\m\n}B_{\m\n}\Big) +2 g g' \l_2 Y_{\Ph} \big(H^{\dag}\t^a H\big) W_{\m\n}^aB_{\m\n} \\
&= -(2\l_1 + \l_2)\Big(\frac{1}{4} \scO_{WW} + Y_{\Ph}^2 \scO_{BB}\Big) + \l_2Y_{\Ph} \scO_{WB} .
\end{align*}

\noindent \textit{Returning to the full Lagrangian}\\

Now we return to the full Lagrangian in~\eqref{eqn:EW_doub_lag} and leave all couplings non-zero. This makes the calculation more complicated; however, it will not be too difficult---we will simply need to evaluate some traces which, while tedious, is very straightforward. In many regards, most of the work goes into setting up the matrix that we are tracing over. %In the present case, with arbitrary couplings in~\eqref{eqn:EW_doub_lag} and the non-zero tree-level piece \(\Ph_c\), the matrix is complicated looking, but with a little effort we can see how it all works out.

To evaluate the one-loop effective action, we expand the action around the solution to the equation of motion, \(\Ph = \Ph_c + \s\). For our desired accuracy of dimension-six operators, it is sufficient to take the lowest order solution of \(\Ph_c\), which, from~\eqref{eqn:doub_Ph_c}, is given by
\[
\Ph_c \approx \et_H \frac{\abs{H}^2}{m^2} \tH \equiv k_c \tH, \quad k_c \equiv \et_H \frac{\abs{H}^2}{m^2}.
\]
Because the interaction \((\tH^{\dag}\Ph)^2\) is holomorphic in \(\Ph\), it is easiest to treat \(\Ph\) and \(\Ph^*\) as separate variables. This is equivalent to splitting \(\Ph\) into its real and imaginary pieces, although more convenient to work with. Then, upon expanding \(\Ph = \Ph_c + \s\) and doing a little algebra, the terms quadratic in \(\s\) are
\begin{equation}
\scL[\Ph_c + \s] \supset \frac{1}{2}\begin{matrix} \begin{pmatrix} \s^{\dag} & \s^T \end{pmatrix} \\ \mbox{} \end{matrix} \begin{pmatrix} P^2-m^2 - A' & -2V \\ -2V^{\dag} & \big(P^T\big)^2-m^2 - A'^T \end{pmatrix} \begin{pmatrix} \s \\ \s^* \end{pmatrix} ,
\label{eqn:doub_matrix}
\end{equation}
where
\begin{align}
A' &= (\l_1 + \x_c)\abs{H}^2 + (\l_2 + \x_c)\tH\tH^{\dag} , \nonumber\\
V &= (\l_3 + \x_c/2)\tH\tH^T , \nonumber\\
\x_c &\equiv -2 \et_{\ph} k_c + \frac{\l_{\Ph}}{2}k_c^2, \ k_c \equiv \et_H\abs{H}^2/m^2.
\label{eqn:doub_matrix_defs}
\end{align}
A few comments:
\begin{itemize}
\item We are treating \(\s\) and \(\s^*\) as separate variables, which is the same procedure as working with the real and imaginary parts of \(\s\).
\item The one-loop effective action is given by
\[
\D S_{\text{eff,1-loop}} = \frac{i}{2} \Tr \log \big( \dots \big) ,
\]
with the matrix in~\eqref{eqn:doub_matrix} inserted into the trace. Note the factor of \(1/2\); we take \(c_s = 1/2\) since we are treating \(\s\) and \(\s^*\) as separate, real variables.
\item The subscript ``\textit{c}'' on \(\x_c\) and \(k_c\) indicates that these terms originate from the background configuration \(\Ph_c\). Note that \(\x_c \sim \# \abs{H}^2 + \# \abs{H}^4\) contains powers of the Higgs field. %\(\x_c\) will only contribute at low orders in the covariant derivative expansion since we are truncating at dimension-six operators.
%\item \textcolor{blue}{As in the triplet scalar example, the one-loop effects of the background configuration \(\Ph_c\ne 0\) can be absorbed into redefinition of the UV Lagrangian parameters, and hence dropped from the matching analysis.}
\end{itemize}

We now use the CDE to compute \(\D S_{\text{eff,1-loop}}\). In the CDE formulas, we take
\begin{equation}
P_{\m} = \begin{pmatrix} P_{\m} & 0 \\ 0 & P_{\m}^T \end{pmatrix}, \quad m^2 = \begin{pmatrix} m^2\mathbf{1}_2 & 0 \\ 0 & m^2\mathbf{1}_2 \end{pmatrix}, \quad U = \begin{pmatrix}  A' & 2V \\ 2V^{\dag} & A'^T \end{pmatrix} ,
\label{eqn:doub_CDE_defs}
\end{equation}
where \(\mathbf{1}_2\) is the \(2\times2\) identity matrix. The effective action is of the form \(\Tr \log \big(-P^2 + m^2 + U\big)\), so that the transformation \(e^{\pm P^{\m}\pd/\pd q^{\m}}\) in Eq.~\eqref{eqn:sum_trans} is still allowed and the CDE proceeds as discussed.

Thus, we can immediately use the universal results in Eq.~\eqref{eqn:CDE_universal_lag} with matrices \(P_{\m}\) and \(U\) defined as above in~\eqref{eqn:doub_CDE_defs}, and all that is left to do is evaluate some traces. %This is straightforward, albeit slightly tedious. Note that,
Since \(\x_c \sim \scO(\abs{H}^2)\), we only need to keep \(\x_c\) for \(\tr \, U\) and \(\tr \, U^2\). When we drop \(\x_c\), the matrix \(A'\) is equal to the matrix \(A\) defined in Eq.~\eqref{eqn:doub_A_def}. Tabulating only dim-6 operators, using the operator definitions in Table~\ref{tbl:operators}, and including a factor of \(1/2\) for convenience, we find
\begin{equation}
\def\arraystretch{1.4}
\begin{array}{rclll}
\frac{1}{2}\tr \, U^{\ } & = & \tr \, A' & \supset & \frac{3}{2} \l_{\Ph}\et_H^2 \, \scO_6/m^4\\
\frac{1}{2} \tr \, U^2 & = & \tr \, A'^2 + 4 \tr \, VV^{\dag} & \supset & -4(3\l_1 + 3\l_2 + \l_3)\et_{H}\et_{\Ph} \, \scO_6/m^2\\
\frac{1}{2}\tr \, U^3 & = & \tr \, A^3 + 6 \tr \, \big(A V V^{\dag} + A^T V^{\dag}V \big) &= & \big(2\l_1^3 + 3\l_1^2\l_2 + 3\l_1\l_2^2+\l_2^3 +12(\l_1+\l_2)\l_3^2\big)\scO_6\\
\frac{1}{2}\tr \big(P_{\m}U\big)^2 & = & \tr \big(P_{\m}A\big)^2 + 4\tr \big(P_{\m}V P_{\m}^TV^{\dag}\big)&=& -\big(4\l_1^2 + 4 \l_1\l_2 + \l_2^2 + 4\l_3^2\big)\scO_H - 2\big(\l_2^2 + 4\l_3^2\big)\scO_R \\
 & & & & \quad - \big(\l_2^2 - 4\l_3^2\big)\scO_T  \\
\frac{1}{2}\tr \, UG_{\m\n}'G_{\m\n}' & = & \tr \, A G_{\m\n}'G_{\m\n}'  &=&  -(2\l_1 + \l_2)\Big(\frac{1}{4} \scO_{WW} + Y_{\Ph}^2 \scO_{BB}\Big) + \l_2 Y_{\Ph} \scO_{WB} \\
\frac{1}{2}\tr \, G'^3 & = & ig^3\tr \, W_{\m\n}W_{\n\s}W_{\s\m}& = & -\frac{3}{2}g^2 \scO_{3W} \\
\frac{1}{2} \tr \big(P_{\m}G_{\m\n}'\big)^2 & = & \frac{g^2}{2} \big(D_{\m}W_{\m\n}^a)^2 +2 g'^2 Y_{\Ph}^2 \big(\pd_{\m}B_{\m\n}\big)^2&=& -g^2 \scO_{2W} -4 g'^2Y_{\Ph}^2 \scO_{2B}\\
\end{array}
\label{eqn:doub_loop_traces}
\end{equation}
Plugging these traces into Eq.~\eqref{eqn:CDE_universal_lag} we obtain the one-loop effective Lagrangian. We summarize the results below.

\begin{center} \small{\textbf{Electroweak scalar doublet summary}} \end{center}

We took an electroweak scalar doublet \(\Ph\) with hypercharge \(Y_\Ph = -1/2\) and Lagrangian
\begin{align}
\scL \supset &\abs{D_{\m}\Ph}^2 - m^2 \abs{\Ph}^2 - \frac{\l_{\Ph}}{4}\abs{\Ph}^4 +\big(\et_H \abs{H}^2+\et_{\ph}\abs{\Ph}^2\big)\big(\Ph\cdot H + \text{h.c}\big) \nonumber\\
&-\l_1\abs{H}^2\abs{\Ph}^2 - \l_2 \abs{\Ph\cdot H}^2 -\l_3 \big[\big(\Ph\cdot H\big)^2 + \text{h.c.} \big],
\label{eqn:EW_doub_lag_sum}
\end{align}
and integrated out \(\Ph\) to find the dimension-six operators of the effective action matched at one-loop order.

The tree-level effective action, given in Eq.~\eqref{eqn:EW_doub_tree}, only contains \(\scO_6 = \abs{H}^6\). The one-loop effective action is obtained from plugging the traces in Eq.~\eqref{eqn:doub_loop_traces} into~\eqref{eqn:CDE_universal_lag}. This piece contains a host of dimension-six operators that affect electroweak and Higgs physics. In summary, the effective Lagrangian at the matching scale is given by
\begin{align}
\scL_{\text{eff}} = \scL_{\text{SM}} &+ \frac{1}{m^2}\bigg(c_6 \scO_6 + c_H \scO_H + c_T \scO_T + c_R \scO_R + c_{BB}\scO_{BB} + c_{WW}\scO_{WW} \nonumber\\ &+ c_{WB}\scO_{WB} + c_{3W}\scO_{3W} +c_{2W}\scO_{2W} + c_{2B}\scO_{2B}\bigg) , %\nonumber
\end{align}
where the Wilson coefficients are given in Table~\ref{tbl:EW_doublet}.% \textcolor{blue}{In our renormalization scheme (MS), there is a finite threshold correction at \(\m = m\) in the \(\tr \, U\) term, which leads to the appearance of \(\Ph\)'s self-coupling in \(c_6\) at one-loop.}

\begin{table}
\centering
\[\renewcommand\arraystretch{1.7}
\begin{array}{|rcl|rcl|rcl|}
\hline
c_H &=& \frac{1}{(4\pi)^2}\cdot \frac{1}{12}\cdot \big( 4\l_1^2 + 4 \l_1\l_2 + \l_2^2 + 4\l_3^2\big)
& c_{BB} &=& \frac{1}{(4\pi)^2} \cdot \frac{1}{12}\cdot Y_\Ph^2(2\l_1+\l_2)
& c_{3W} &=& \frac{1}{(4\pi)^2} \cdot \frac{1}{60}\cdot g^2
\\
c_T &=& \frac{1}{(4\pi)^2}\cdot\frac{1}{12} \cdot \big(\l_2^2-4\l_3^2\big)
& c_{WW} &=& \frac{1}{(4\pi)^2} \cdot \frac{1}{48} \cdot (2\l_1+\l_2)
& c_{2W} &=& \frac{1}{(4\pi)^2} \cdot \frac{1}{60}\cdot g^2
\\
c_R &=& \frac{1}{(4\pi)^2}\cdot\frac{1}{6}\cdot \big(\l_2^2+4\l_3^2\big)
& c_{WB} &=& - \frac{1}{(4\pi)^2} \cdot \frac{1}{12}\cdot \l_2 Y_\Ph
& c_{2B} &=& \frac{1}{(4\pi)^2} \cdot \frac{1}{60}\cdot 4g'^2Y_\Ph^2
\\
\hline
\end{array}
\]
\[
\begin{array}{|l|}
\hline
c_6 = \et_{H}^2 + \frac{1}{(4\pi)^2}\cdot \bigg[-\frac{3}{2} \l_{\Ph}\et_H^2 -\frac{1}{6}\big( 2\l_1^3 + 3\l_1^2\l_2 + 3\l_1\l_2^2+\l_2^3\big) -2\big(\l_1+\l_2\big)\l_3^2\bigg]\\
\hline
\end{array}
\]
\vspace{-15pt}
\caption{\label{tbl:EW_doublet}  Wilson coefficients \(c_i\) for the operators \(\scO_i\) in Table~\ref{tbl:operators} generated from integrating out a massive electroweak scalar doublet \(\Ph\) with hypercharge \(Y_{\Ph} = -1/2\). \(g\) and \(g'\) denote the gauge couplings of \(SU(2)_L\) and \(U(1)_Y\), respectively. The couplings \(\l_{1,2,3}\) and \(\et_{\Ph,H}\) are defined by the Lagrangian in Eq.~\eqref{eqn:EW_doub_lag_sum}; they are associated with various interactions between \(\Ph\) and the SM Higgs doublet \(H\).}
\vspace{-5pt}
\end{table}
\renewcommand\arraystretch{1.0}

\subsubsection{A $SU(2)_L$ quartet scalar}

In this example, we consider a heavy complex $SU(2)_L$ quartet scalar $\Phi$ with mass $m$ and SM hypercharge $Y_\Phi=\frac{3}{2}$. \textcolor{blue}{An allowed \(\Phi H^3\) coupling to the Higgs leads to tree-level contributions in the effective action. For brevity, we will ignore other interaction terms with the Higgs, \textit{e.g.} \(\abs{\Ph}^2\abs{H}^2\), as well as the quartet's self-couplings---they can be easily included as in previous examples. This amounts to taking \(U =0\) in Eq.~\ref{eqn:CDE_universal_lag}. Thus, we consider the following Lagrangian}
\begin{equation}
\Delta \mathcal{L} = {\Phi ^\dag }\left( - {D^2} - {m^2}\right)\Phi  - \left(\Phi^\dag B + c.c.\right) , \label{eqn:Lquartet}
\end{equation}
where $\Phi=\left(\Phi_1,\Phi_2,\Phi_3,\Phi_4\right)^T$, with each component being eigenstate of the third $SU(2)_L$ generator $t_\Phi^3=\text{diag}\left(\frac{3}{2}, \frac{1}{2},-\frac{1}{2},-\frac{3}{2}\right)$, and \(B\sim H^3\). Specifically,
\begin{equation}
B = \left( {\begin{array}{*{20}{c}}
{H_1^3}\\
{\sqrt 3 H_1^2{H_2}}\\
{\sqrt 3 {H_1}H_2^2}\\
{H_2^3}
\end{array}} \right) ,
\end{equation}
where $H_1$ and $H_2$ are components of the SM Higgs field $H=(H_1,H_2)^T$.\footnote{\textcolor{blue}{Similarly, for quartet scalar $\Phi$ with $Y_\Phi=1/2$, $B$ would be given by}
\begin{equation}
B_{Y=1/2} = \left( {\begin{array}{*{20}{c}}
{H_1^2 {\tilde H}_1}\\
{\frac{1}{\sqrt 3} H_1^2{\tilde H}_2 + \frac{2}{\sqrt 3} H_1H_2{\tilde H}_1}\\
{\frac{1}{\sqrt 3} H_2^2{\tilde H}_1 + \frac{2}{\sqrt 3} H_1H_2{\tilde H}_2}\\
{H_2^2 {\tilde H}_2}
\end{array}} \right) .
\end{equation}
}

Again, we follow the procedure described in Section~\ref{sec:CDE_tree} to compute the tree-level effective Lagrangian. We first get the equation of motion
\begin{equation}
\left(-D^2-m^2\right)\Phi_c = B , \nonumber
\end{equation}
which gives the solution
\begin{equation}
\Phi_c = -\frac{1}{D^2+m^2} B \approx -\frac{1}{m^2} B . \nonumber
\end{equation}
Plugging this solution back to Eq.~\eqref{eqn:Lquartet}, we get
\begin{equation}
\Delta \mathcal{L}_\text{eff,tree} = -B^\dag \Phi_c \approx \frac{1}{m^2} B^\dag B = \frac{1}{m^2}\left|H\right|^6 = \frac{1}{m^2}\mathcal{O}_6 .
\end{equation}

Because we are ignoring other interactions that \(\Ph\) may have, at one-loop we only get dimension-six operators solely involving gauge fields. The general contribution of particles to the pure glue Wilson coefficients was given in Table~\ref{tbl:dim6_pureglue}. The quartet is the spin \(3/2\) representation of \(SU(2)\) and has Dynkin index \(\m(R) = 5\). Therefore, for \(\scO_{2W}\) and \(\scO_{3W}\), we find
\begin{equation}
\D \scL_{\text{eff,1-loop}} \supset \frac{1}{(4\pi)^2} \frac{1}{m^2}\, \frac{g^2}{6} \big( \scO_{2W} + \scO_{3W} \big).
\end{equation}
For abelian gauge groups we can also use the results of Table~\ref{tbl:dim6_pureglue}: replace \(a_{2s}\m(R)\) with \(n_{\Ph}Q^2\), where \(Q\) is the charge of \(\Ph\) under the abelian group and \(n_{\ph}\) is the number of real-degrees of freedom in \(\Ph\). (Note that, by anti-symmetry on the Lorentz indices, \(\scO_{3G}\) vanishes if the group is abelian.)  For the case at hand, the quartet has hypercharge \(3/2\) and four complex (eight real) degrees of freedom. Therefore,
\begin{equation}
\D \scL_{\text{eff,1-loop}} \supset \frac{1}{(4\pi)^2} \frac{1}{m^2}\, \frac{3}{10}\, g'^2\scO_{2B}.
\end{equation}

%Next let us compute the 1-loop piece of the effective Lagrangian, which according to Eq.~\eqref{eqn:Seff_realscalar}, is
%\begin{equation}
%\Delta S_\text{eff,1-loop} = 4i\text{Tr}\log\left(D^2 + m^2\right) .
%\end{equation}
%Clearly, this is again in the form of Eq.~\eqref{eqn:sum_seff}, with
%\begin{eqnarray}
%U &=& 0 , \\
%G'_{\mu\nu} &=& [D_\mu, D_\nu] = -igW_{\mu\nu}^a t_\Phi^a - ig'B_{\mu\nu} Y_\Phi .
%\end{eqnarray}
%Useful traces related are
%\begin{eqnarray}
%\tr{({D^\mu }{G'_{\mu\nu}})^2} &=& - {g^2}({D^\mu }W_{\mu \nu }^a)({D_\rho }{W^{b\rho \nu }})\tr(t_\Phi ^at_\Phi ^b) - {{g'}^2}{({\partial ^\mu }{B_{\mu \nu }})^2}\tr(Y_\Phi ^2) \nonumber \\
% &=&  - 5{g^2}{({D^\mu }W_{\mu \nu }^a)^2} - 9{{g'}^2}{({\partial ^\mu }{B_{\mu \nu }})^2} \nonumber \\
% &=& 10{g^2}{\mathcal{O}_{2W}} + 18{{g'}^2}{\mathcal{O}_{2B}} , \\
%\tr(G_\mu'^\nu G_\nu'^\rho G_\rho'^\mu) &=& i{g^3}W_\mu ^{a\nu }W_\nu ^{b\rho }W_\rho ^{c\mu }\tr(t_\Phi ^at_\Phi ^bt_\Phi ^c) \nonumber \\
% &=& i{g^3}W_\mu ^{a\nu }W_\nu ^{b\rho }W_\rho ^{c\mu }\frac{5}{2}i{\epsilon^{abc}} \nonumber \\
% &=&  - 15{g^2}{\mathcal{O}_{3W}} .
%\end{eqnarray}
%Putting them all together into Eq.~\eqref{eqn:CDE_universal_lag}, we obtain
%\begin{eqnarray}
%\Delta {\mathcal{L}_{{\rm{eff,1 - loop}}}} &=& \frac{1}{{{{(4\pi )}^2}}}\frac{1}{{{m^2}}}\tr\left[ { - \frac{1}{{60}}{{\left({P^\mu }{G'_{\mu\nu}}\right)}^2} - \frac{1}{{90}}G_\mu'^\nu G_\nu'^\rho G_\rho'^\mu} \right] \nonumber \\
% &=& \frac{1}{{{{(4\pi )}^2}}}\frac{1}{{{m^2}}}\left[ {\frac{1}{{60}}\left(10{g^2}{\mathcal{O}_{2W}} + 18{{g'}^2}{\mathcal{O}_{2B}}\right) - \frac{1}{{90}}\left( - 15{g^2}{\mathcal{O}_{3W}}\right)} \right] \nonumber \\
% &=& \frac{1}{{{{(4\pi )}^2}}}\frac{1}{{{m^2}}}\left(\frac{1}{6}{g^2}{\mathcal{O}_{3W}} + \frac{1}{6}{g^2}{\mathcal{O}_{2W}} + \frac{3}{{10}}{{g'}^2}{\mathcal{O}_{2B}}\right) .
%\end{eqnarray}

\subsubsection{A real singlet scalar}

In this example, we consider a heavy real singlet scalar field $\Phi$ with mass $m$ that couples to the SM through the following Lagrangian
\begin{equation}
\Delta \mathcal{L} = \frac{1}{2} \left(\partial_\mu \Phi\right)^2 - \frac{1}{2} m^2 \Phi^2 -A \left| H \right|^2 \Phi - \frac{1}{2} k\left| H \right|^2 \Phi^2 - \frac{1}{3!}\mu \Phi^3 -\frac{1}{4!}\lambda_\Phi \Phi^4 . \label{eqn:LSinglet}
\end{equation}
Integrating out this heavy scalar $\Phi$ generates a SM EFT that matches the above UV theory at the scale $\Lambda=m$. We previously computed the tree-level Wilson coefficients in~\cite{Henning:2014gca}; here we demonstrate how to perform this calculation as well as provide the one-loop values of the Wilson coefficients. We note that this real scalar can have interesting phenomenological consequences, such as generating a first order EW phase transition~\cite{Grojean:2004xa}; see the discussion and references in~\cite{Henning:2014gca}.

To compute the tree-level effective Lagrangian we follow the procedure described in Section~\ref{sec:CDE_tree}, taking \(P_{\m} = i \pd_{\m}\). %we first obtain the equation of motion
%\begin{equation}
%\left(\partial^2 + m^2 + k\left| H \right|^2\right)\Phi + \frac{1}{2}\mu \Phi^2 + \frac{1}{3!}\lambda_\Phi \Phi^3 = -A\left| H \right|^2 , \nonumber
%\end{equation}
%which gives the solution
The solution to the linearized equation of motion is,
\begin{equation}
\Phi_c \approx - \frac{1}{\partial^2 + m^2 + k\left| H \right|^2} A\left| H \right|^2 \approx -\frac{1}{m^2} A\left| H \right|^2 + \frac{1}{m^4}\left(\partial^2 + k\left| H \right|^2\right) A\left| H \right|^2 . \nonumber
\end{equation}
Plugging this solution back to Eq.~\eqref{eqn:LSinglet}, we get the tree-level effective Lagrangian
\begin{eqnarray}
\Delta \mathcal{L}_\text{eff,tree} &=&  -A\left| H \right|^2 \Phi_c + \frac{1}{2}\Phi_c\left( -\partial^2 - m^2 - k\left| H \right|^2\right) \Phi_c - \frac{1}{3!}\mu \Phi_c^3 - \frac{1}{4!}\lambda_\Phi \Phi_c^4 \nonumber \\
 %&=& -\frac{1}{2}A\left| H \right|^2 \Phi_c -\frac{1}{3!}\mu \Phi_c^3 - \frac{1}{4!}\lambda_\Phi \Phi_c^4 \nonumber \\
 &\approx& \frac{1}{2m^2} A^2\left| H \right|^4 + \frac{A^2}{m^4}\mathcal{O}_H + \left( -\frac{kA^2}{2m^4} + \frac{1}{3!}\frac{\mu A^3}{m^6}\right)\mathcal{O}_6 .
\end{eqnarray}

Next let us compute the 1-loop piece of the effective Lagrangian, which according to Eq.~\eqref{eqn:Seff_realscalar}, is
\begin{eqnarray}
\Delta S_\text{eff,1-loop} &=& \frac{i}{2}\text{Tr}\log\left( -{\left. {\frac{{{\delta ^2}S}}{{\delta {\Phi ^2}}}} \right|_{{\Phi _c}}}\right) = \frac{i}{2}\text{Tr}\log\left({\partial ^2} + {m^2} + k{\left| H \right|^2} + \mu {\Phi _c} + \frac{1}{2}{\lambda _\Phi }\Phi _c^2\right) \nonumber \\
 &=& \frac{i}{2}\text{Tr}\log\left({\partial ^2} + {m^2} + k{\left| H \right|^2}\right) = \frac{i}{2}\text{Tr}\log\left( - {P^2} + {m^2} + U\right) .
\end{eqnarray}
This is clearly in a form of Eq.~\eqref{eqn:sum_seff}, with $U=k\left|H\right|^2$ and $G'_{\mu\nu}=[D_\mu, D_\nu]=[\partial_\mu, \partial_\nu]=0$. Plugging these specific values of $U$ and $G'_{\mu\nu}$ into Eq.~\eqref{eqn:CDE_universal_lag}, we obtain
\begin{eqnarray}
\Delta {\mathcal{L}_\text{eff,1-loop}} &=& \frac{1}{{2{{(4\pi )}^2}}}\frac{1}{{m^2}}\left[ { - \frac{1}{{12}}{{\left({P_\mu }U\right)}^2} - \frac{1}{6}U^3} \right] \nonumber \\
 &=& \frac{1}{{2{{(4\pi )}^2}}}\frac{1}{{m^2}}\left[ {\frac{{{k^2}}}{{12}}{{\left({\partial _\mu }{{\left| H \right|}^2}\right)}^2} - \frac{{{k^3}}}{6}{{\left| H \right|}^6}} \right] \nonumber \\
 &=& \frac{1}{{{{(4\pi )}^2}}}\frac{1}{{m^2}}\left(\frac{{{k^2}}}{{12}}{\mathcal{O}_H} - \frac{{{k^3}}}{{12}}{\mathcal{O}_6}\right) .
\end{eqnarray}

\subsubsection{Supersymmetry and light scalar tops}
Supersymmetric states at or near the electroweak scale could explain the origin of this scale and its radiative stability. Scalar tops (stops) hold a privileged position in providing a natural explanation to origin of the EW scale. This motivated us in a previous work~\cite{Henning:2014gca} to study the low-energy EFT that results when stops are integrated out. In that work, we considered a supersymmetric spectrum with light stops and other superpartners decoupled and computed the Wilson coefficients of the one-loop effective action. In this paper, we provide more details of how the Wilson coefficients are calculated using the covariant derivative expansion.

As stops carry all SM gauge quantum numbers, every operator in Table~\ref{tbl:operators} is generated. In~\cite{Henning:2014gca}, we computed the Wilson coefficients separately using the CDE and traditional Feynman diagram techniques. The results agreed, providing a good consistency check of the calculation.\footnote{A recent paper by Craig \textit{et al.} \cite{Craig:2014una} computed the correction from scalar tops to the \(Zh\) associated production cross section $\sigma_{Zh}^{}$. They compared the result of the full NLO calculation versus the Wilson coefficients from the SM EFT. Excellent agreement was found, which also serves as a good consistency check.} More importantly, however, the two methods highlighted just how much effort the CDE saves over traditional techniques. No doubt the CDE computation is still complicated, as we will see below, but that is because stops have a large number of various interactions with the SM Higgs and gauge bosons. Nevertheless, it is extremely systematic.

We integrate out the multiplet $\Phi=(\tilde{Q}_3,{\tilde t}_R)^T$, the Lagrangian of which up to quadratic order is given by
\begin{equation}
\mathcal{L} = \Phi^\dagger \left( -D^2-m^2-U \right) \Phi ,
\end{equation}
where
\begin{equation}
{m^2} = \left( {\begin{array}{*{20}{c}}
{m_{{{\tilde Q}_3}}^2}&0\\
0&{m_{{{\tilde t}_R}}^2}
\end{array}} \right) ,
\end{equation}
and the matrix $U$ is
\begin{align*}
U &= \begin{pmatrix} \big(y_t^2s_{\b}^2 + \frac{1}{2}g^2c_{\b}^2\big)\tH\tH^{\dag} + \frac{1}{2} g^2 s_{\b}^2HH^{\dag} - \frac{1}{2}\big(g'^2 Y_Q c_{2\b} + \frac{1}{2}g^2\big) \abs{H}^2 & y_t s_{\b} X_t \tH \\
y_t s_{\b} X_t \tH^{\dag} & \big( y_t^2s_{\b}^2 - \frac{1}{2} g'^2 Y_{t_r} c_{2\b}\big) \abs{H}^2 \end{pmatrix} \\
&\equiv \begin{pmatrix} \tk \tH\tH^{\dag} + kH H^{\dag} + \l_L \abs{H}^2 & X_t \tH \\ X_t \tH^{\dag} & \l_R \abs{H}^2 \end{pmatrix} \\
&\equiv \begin{pmatrix} A_L & X_t \tH \\ X_t\tH^{\dag} & A_R \end{pmatrix}
\end{align*}
where we have defined
\[
\def\arraystretch{1.5}
\begin{array}{ccc}
A_L \equiv \tk \tH\tH^{\dag} + kH H^{\dag} + \l_L \abs{H}^2 \hspace{3mm} & A_R \equiv \l_R \abs{H}^2 \hspace{3mm} & y_ts_{\b} X_t \to X_t  \\
\tk \equiv y_t^2s_{\b}^2 + \frac{1}{2}g^2c_{\b}^2 & k \equiv \frac{1}{2} g^2 s_{\b}^2 & \l_L \equiv - \frac{1}{2}\big(g'^2 Y_Q c_{2\b} + \frac{1}{2}g^2\big) \\
\l_R \equiv y_t^2s_{\b}^2 - \frac{1}{2} g'^2 Y_{t_r} c_{2\b} & & \\
\end{array}
\]
Now with both the representation and the interaction matrix $U$ at hand, we are ready to make use of Eq.~\eqref{eqn:CDE_universal_lag} to compute the Wilson coefficients. However, in order for Eq.~\eqref{eqn:CDE_universal_lag} to be valid, we need $U$ to commute with the mass square matrix $m^2$, which limits us to the degenerate mass scenario $m_{{\tilde Q}_3}^2=m_{{\tilde t}_R}^2\equiv m_{\tilde t}^2$. It is also worth noting that due to the appearance of $X_t$, $U$ is no long quadratic in $H$, but also contains linear term of $H$. This means that one has to keep up to $\mathcal{O}(U^6)$ in computing the Wilson coefficients of dimension-six operators. Another thing to keep in mind while evaluating the terms in Eq.~\eqref{eqn:CDE_universal_lag} is that ${\tilde Q}_3$ and ${\tilde t}_R$ have different charges under the SM gauge group, and the covariant derivative $D_\mu$ or $P_\mu=iD_\mu$ should take on the appropriate form for each.
\[
P_{\m} = \begin{pmatrix} P_{L\m} & 0 \\ 0 & P_{R\m} \end{pmatrix}
\]
For example, the commutator $[P_\mu,U]$ is
\[
[P_{\m},U] = \begin{pmatrix} [P_{L\m},A_L] & X_t (P_{\m}\tH) \\ X_t (P_{\m}\tH)^{\dag} & [P_{R\m},A_R] \end{pmatrix}
\]
Through a straightforward, albeit tedious, use of Eq.~\eqref{eqn:CDE_universal_lag}, we obtain the final result of Wilson coefficients listed in Table~\ref{tbl:MSSM}.


\begin{table}\renewcommand\arraystretch{1.5}
\centering
{\footnotesize
\input{./tbl_mssm_tikz.tex}
}
\vspace{-15pt}
\caption{\label{tbl:MSSM}  Wilson coefficients \(c_i\) for
  the operators \(\scO_i\) in Table~\ref{tbl:operators} generated
  from integrating out MSSM stops with degenerate soft mass
  \(\mt\). \(g_s,g,\) and \(g'\) denote the gauge couplings of
  \(SU(3),SU(2)_L,\) and \(U(1)_Y\), respectively, \(h_t = m_t/v\) with $v=174GeV$,
  and \(\tan \b = \langle
  H_u\rangle / \langle H_d \rangle\) in the MSSM.}
\vspace{-5pt}
\end{table}
\renewcommand\arraystretch{1.0}

\subsubsection{Kinetic mixing of gauge bosons}

In this example, we consider a heavy $U(1)$ gauge boson $K_\mu$ with mass $m_K$ that has a kinetic mixing with the SM $U(1)_Y$ gauge boson $B_\mu$ through
\begin{equation}
\Delta\mathcal{L} = - \frac{1}{4}{K_{\mu \nu }}{K^{\mu \nu }} + \frac{1}{2}m_K^2{K_\mu }{K^\mu } - \frac{k}{2}{B^{\mu \nu }}{{K}_{\mu \nu }} , \label{eqn:Lmixing}
\end{equation}
where $K_{\mu\nu}$ denotes the field strength $K_{\mu\nu}=\partial_\mu K_\nu -\partial_\nu K_\mu$. Again, the tree-level effective Lagrangian can be obtained by following the procedure described in Section~\ref{sec:CDE_tree}. We first find the equation of motion of this heavy gauge boson $K_\mu$
\begin{equation}
{\partial _\nu }{K^{\mu \nu }} + k({\partial _\nu }{B^{\mu \nu }}) = m_K^2{K^\mu } , \nonumber
\end{equation}
which, as usual for vector bosons, can be decomposed into two equations
\begin{eqnarray}
{\partial _\mu }{K^\mu } &=& 0 , \nonumber \\
\left( -\partial^2 - m_K^2\right){K^\mu } &=&  - k({\partial _\nu }{B^{\mu \nu }}) . \nonumber
\end{eqnarray}
Solving these, we get the classical solution
\begin{equation}
{K_{c\mu} } = \frac{k}{{{\partial ^2} + m_K^2}}({\partial ^\nu }{B_{\mu \nu }}) \approx \frac{k}{{m_K^2}}({\partial ^\nu }{B_{\mu \nu }}). \label{eqn:mixingsolution}
\end{equation}
Next we plug this solution back into the UV model Lagrangian (Eq.~\eqref{eqn:Lmixing}) to get the tree-level effective Lagrangian. With ${B^{\mu \nu }}{K_{\mu \nu }} = 2({\partial _\nu }{B^{\mu \nu }}){K_\mu }$, we obtain
\begin{eqnarray}
\Delta\mathcal{L}_\text{eff,tree} &=& - \frac{1}{2}{K_{c\mu} }\left[ {\left( - {\partial ^2} - m_K^2\right){g^{\mu \nu }} + {\partial ^\mu }{\partial ^\nu }} \right]{K_{c\nu} } - \frac{k}{2}{B^{\mu \nu }}{K_{c\mu \nu }} \nonumber \\
 &=&  \frac{k}{2}({\partial _\nu }{B^{\mu \nu }}){K_{c\mu} } - k({\partial _\nu }{B^{\mu \nu }}){K_{c\mu} } \nonumber \\
 &=& -\frac{k}{2}({\partial _\nu }{B^{\mu \nu }}){K_{c\mu} } \nonumber \\
 &=&  \frac{{{k^2}}}{{m_K^2}}{\mathcal{O}_{2B}}. \label{eqn:mixingresult}
\end{eqnarray}
Note that this example has a trivial one-loop contribution to the effective action.

\subsubsection{A heavy $SU(2)$ gauge boson}

\textcolor{blue}{Here we consider an example involving heavy gauge bosons. Heavy vector bosons generically arise in, for example, extra-dimensional compactifications}~\cite{Manton:1979kb} \textcolor{blue}{and little Higgs theories}~\cite{ArkaniHamed:2002qx,*ArkaniHamed:2002qy}. \textcolor{blue}{We note that this covariant EFT calculation of the one-loop effective action provides great simplification to the traditional loop calculation involving massive vector bosons. For example, this method could be readily employed to study massive vector bosons whose tree-level contributions are absent due to, \textit{e.g.}, KK-parity}~\cite{Cheng:2002iz} \textcolor{blue}{in extra-dimensional models or T-parity}~\cite{Cheng:2003ju,*Cheng:2004yc} \textcolor{blue}{in little Higgs models. }%Frequently, these massive vector bosons modify SM processes at tree-level (see, \textit{e.g.},~\cite{Perelstein:2005ka}).

We consider an $SU(2)_1\times SU(2)_2$ gauge symmetry where with a scalar \(\Ph\) transforming as a bifundamental. We take the Standard Model fermions and Higgs field to be localized to the \(SU(2)_1\) gauge group. (We suppress color and hypercharge; the full gauge symmetry is \(SU(2)_1\times SU(2)_2 \times U(1)_Y \times SU(3)_c\).) The scalar \(\Ph\) takes a vev, breaking the \(SU(2)\) groups down to their diagonal subgroup, which we identify with the weak interactions of the SM, \(SU(2)_1 \times SU(2)_2 \to SU(2)_L\). This is simply a deconstructed~\cite{ArkaniHamed:2001nc} version of an extra-dimensional model (\textit{e.g.} \cite{Randall:1999ee}), where the weak gauge bosons, being a diagonal combination of the \(SU(2)_1\times SU(2)_2\) gauge bosons, ``propagate in the bulk'', while the SM fermions and Higgs only transform under one gauge group and are therefore ``localized''.

The relevant kinetic terms of the Lagrangian are
\begin{equation}
\Delta \mathcal{L}_K = - \frac{1}{2}\tr{\big(F_1^{\mu\nu}\big)^2} - \frac{1}{2}\tr{\big(F_2^{\mu\nu}\big)^2} + \frac{1}{2}\tr{({\mathcal{D}_\mu }\Ph )^\dag }({\mathcal{D}^\mu }\Ph ) ,
\end{equation}
where the scalar $\Ph$ transforms as a bifundamental, $\Ph \to U_1 \Ph U_2^\dag$. The covariant derivative of the UV theory is given by\footnote{Note that the action of \(\mathcal{D}_{\m}\) on \(\Ph\) is \(\mathcal{D}_{\m}\Ph = \pd_{\m}\Ph - i g_1 A_{1\, \m}\Ph + i g_2 \Ph A_{2\, \m}\)}
\[
\mathcal{D}_{\m} = \pd_{\m} - i g_1 A_{1\, \m} - i g_2A_{2\, \m},
\]
where \(g_i\) and \(A_{i\, \m} = A_{i\, \m}^a\t_i^a\) are the gauge coupling and gauge bosons of the \(SU(2)_i\) with the generators \(\t_i^a\) taken in the fundamental representation. A vacuum expectation value for \(\Ph\),
\[
\avg{\Ph} = \frac{1}{\sqrt{2}}\begin{pmatrix} v& 0\\0 & v \end{pmatrix},
\]
breaks $SU{(2)_1} \times SU{(2)_2} \to SU{(2)_L}$. % upon taking a vev as
%\begin{equation}
%\Ph  = \frac{1}{{\sqrt 2 }}(v + h) \begin{pmatrix} 1& 0\\0 & 1 \end{pmatrix} + i\sqrt 2 {\chi ^a}{t^a} .
%\end{equation}
The mass eigenstates are
\begin{eqnarray}
{Q^a} &\equiv& \frac{1}{{\sqrt {g_1^2 + g_2^2} }}({g_1}A_1^a - {g_2}A_2^a) , \\
{W^a} &\equiv& \frac{1}{{\sqrt {g_1^2 + g_2^2} }}({g_2}A_1^a + {g_1}A_2^a) ,
\end{eqnarray}
where $W^a$ are the SM gauge bosons corresponding to the unbroken symmetry $SU(2)_L$, and $Q^a$ obtain a mass \(m_Q^2 = (g_1^2+g_2^2)v^2/4\) from the Higgs mechanism. \(Q_{\m}\) transforms in the adjoint of the unbroken \(SU(2)_L\).

In terms of the mass eigenstates, the covariant derivative becomes
\begin{equation}
{\mathcal{D}_\mu } = {\partial _\mu } - igW_\mu ^a\t_L^a - iQ_\mu ^a\bigg(\frac{{g_1^2}}{{\sqrt {g_1^2 + g_2^2} }}\t_1^a - \frac{{g_2^2}}{{\sqrt {g_1^2 + g_2^2} }}\t_2^a\bigg) ,
\end{equation}
where \(\t_L^a = \t_1^a + \t_2^a\) are the unbroken generators and we identify $g \equiv g_1g_2/\sqrt {g_1^2 + g_2^2}$ as the weak coupling constant of the SM. We expand \(\Ph\) around \(\avg{\Ph}\),
\begin{equation}
\Ph  = \frac{1}{{\sqrt 2 }}(v + h) \begin{pmatrix} 1& 0\\0 & 1 \end{pmatrix} + i\sqrt 2 {\chi ^a}{\t^a} .
\end{equation}
where the \(\chi^a\) are the Nambu-Goldstone bosons transforming in the adjoint of the unbroken \(SU(2)_L\) and \(h\) is the massive Higgs field.

Expanding out $\mathcal{L}_K$ in terms of $W_\mu$, $Q_\mu$, $\chi$, and adding with the gauge fixing piece $\mathcal{L}_\text{g.f.}$, the ghost term $\mathcal{L}_\text{ghost}$, as well as the interaction $\mathcal{L}_\text{I}$ between $Q_\mu$ and the SM fields
\begin{eqnarray}
\Delta \mathcal{L}_K &\supset& - \frac{1}{2}\tr{({D^\mu }{Q^\nu } - {D^\nu }{Q^\mu })^2} + ig\tr([{Q^\mu },{Q^\nu }]{W_{\mu \nu }}) + \tr{({D_\mu }\chi - {m_Q}{Q_\mu })^2} , \\
{\mathcal{L}_\text{g.f.}} &=&  - \frac{1}{\xi }\tr{(\xi {m_Q}\chi  + {D^\mu }{Q_\mu })^2} , \\
{\mathcal{L}_\text{ghost}} &\supset& {{\bar c}^a}{( - {D^2} - \xi m_Q^2)^{ab}}{c^b} , \\
{\mathcal{L}_\text{I}} &=& \frac{{g_1^4}}{{4(g_1^2 + g_2^2)}}{\left| H \right|^2}Q_\mu ^a{Q^{a\mu }} + \frac{{g_1^2}}{\sqrt{g_1^2 + g_2^2}}Q_\mu ^aJ_W^{a\mu} ,
\end{eqnarray}
we get the full Lagrangian up to quadratic terms in $Q_\mu^a$ as
\begin{eqnarray}
\Delta \mathcal{L} &=& \frac{1}{2}Q_\mu ^a{\left\{ {{D^2}{g^{\mu \nu }} - {D^\nu }{D^\mu } + m_Q^2{g^{\mu \nu }} + [{D^\mu },{D^\nu }] + \frac{1}{\xi }{D^\mu }{D^\nu } + \frac{{g_1^4}}{{2(g_1^2 + g_2^2)}}{{\left| H \right|}^2}} g^{\mu\nu} \right\}^{ab}}Q_\nu ^b \nonumber \\
 && + \frac{{g_1^2}}{{\sqrt {g_1^2 + g_2^2} }}Q_\mu ^aJ_W^{a\mu } + \frac{1}{2}{\chi ^a}{( - {D^2} - \xi m_Q^2)^{ab}}{\chi ^b} + {{\bar c}^a}{( - {D^2} - \xi m_Q^2)^{ab}}{c^b} ,
\end{eqnarray}
where $H$ denotes the SM Higgs field, and $J_W^{a\mu}$ is the source current of the SM $W_\mu^a$. Working with Feynman gauge $\xi=1$, we get
\begin{eqnarray}
\Delta \mathcal{L} &=& \frac{1}{2}Q_\mu ^a{\left\{ {{D^2}{g^{\mu \nu }} + m_Q^2{g^{\mu \nu }} + 2[{D^\mu },{D^\nu }] + \frac{{g_1^4}}{{2(g_1^2 + g_2^2)}}{{\left| H \right|}^2}} g^{\mu\nu} \right\}^{ab}}Q_\nu ^b \nonumber \\
 && + \frac{{g_1^2}}{{\sqrt {g_1^2 + g_2^2} }}Q_\mu ^aJ_W^{a\mu } + \frac{1}{2}{\chi ^a}{( - {D^2} - m_Q^2)^{ab}}{\chi ^b} + {{\bar c}^a}{( - {D^2} - m_Q^2)^{ab}}{c^b} . \label{eqn:LSU2}
\end{eqnarray}
This Lagrangian is clearly in the form of Eq.~\eqref{eqn:Sgauge}, supplemented by a linear interaction term.

Although the heavy fields $Q_\mu^a$ couple directly to the fermions in SM, upon using equation of motion, the tree-level effective Lagrangian turns out to contain only bosonic operators. To see this, let us first solve the equation of motion at leading order
\begin{equation}
Q_c^{a\mu} =  - \frac{{g_1^2}}{{\sqrt {g_1^2 + g_2^2} }}\frac{1}{{m_Q^2}}J_W^{a\mu } .
\end{equation}
Then we plug it back to Eq.~\eqref{eqn:LSU2} and obtain the tree-level effective Lagrangian
\begin{equation}
\Delta {\mathcal{L}_{{\text{eff,tree}}}} = \frac{1}{2}\frac{{g_1^2}}{{\sqrt {g_1^2 + g_2^2} }}Q_\mu ^aJ_W^{a\mu } =  - \frac{1}{{2m_Q^2}}\frac{{g_1^4}}{{g_1^2 + g_2^2}}J_{W\mu }^aJ_W^{a\mu } = \frac{{g_1^4}}{{g_1^2 + g_2^2}}\frac{1}{{m_Q^2}}{\mathcal{O}_{2W}} .
\end{equation}

The one-loop effective Lagrangian can be read off from Table~\ref{tbl:dim6_pureglue} and Eq.~\eqref{eqn:CDE_universal_lag}, with $M^{\mu\nu} = \frac{g_1^4}{2(g_1^2+g_2^2)}{\left| H \right|^2}g^{\mu\nu}$:
\begin{eqnarray}
\Delta {\mathcal{L}_{{\rm{eff,1 - loop}}}} &=& \frac{1}{{{{(4\pi )}^2}}}\frac{1}{{m_Q^2}}\Bigg[ \frac{{{g^2}}}{{20}}\left( {3{\mathcal{O}_{3W}} - 37{\mathcal{O}_{2W}}} \right) + \frac{1}{4}{{\left( {\frac{{g_1^4}}{{g_1^2 + g_2^2}}} \right)}^2}{\mathcal{O}_H} \nonumber \\
 && - \frac{1}{{24}}{{\left( {\frac{{g_1^4}}{{g_1^2 + g_2^2}}} \right)}^3}{\mathcal{O}_6} \Bigg] .
\end{eqnarray}




==> tbl_doublet_tikz.tex <==
%\renewcommand\arraystretch{1.7}
%\begin{table*}[b]
%\caption{\label{tbl:MSSM}  Wilson Coefficients from MSSM stops.}
%\centering
\begin{tikzpicture}[>=latex]
%\draw[help lines] (-4,-4) grid (4,4);
\begin{scope}[xshift=.7cm, yshift = -3.4cm]
\node[anchor=east] at (0,0) {
\scalebox{1.1}{
\begin{tabular}{|rcl|}
  \hline
  \(c_{3G}^{}\) &\(=\)& \(\frac{g_s^2}{(4\pi )^2}\frac{1}{20}\) \\
  \(c_{3W}^{}\) &\(=\)& \(\frac{g^2}{(4\pi)^2}\frac{1}{20}\)  \\
  \(c_{2G}^{}\) &\(=\)& \(\frac{g_s^2}{(4\pi )^2}\frac{1}{20}\) \\
  \(c_{2W}^{}\) &\(=\)& \(\frac{g^2}{(4\pi)^2}\frac{1}{20}\)  \\
  \(c_{2B}^{}\) &\(=\)& \(\frac{g'^2}{(4\pi)^2}\frac{1}{20}\)  \\
  \hline
\end{tabular}
}
};
\end{scope}
%%%%%%%%%%%%% C_GG , c_WB, etc
\begin{scope}[xshift=-1.cm]
\node[anchor=west] at (0,0) {
\scalebox{1.1}{
\begin{tabular}{|rcl|rcl|}
  \hline
  \(c_{GG}^{}\) &\(=\)& \(\frac{h_t^2}{(4\pi)^2} \frac{1}{12} \left[ \left( 1 + \frac{1}{12}\frac{g'^2c_{2\b} }{h_t^2} \right) - \frac{1}{2}\frac{X_t^2}{\mt^2} \right]\) &
  \(c_{WB}^{}\) &\(=\)& \(-\frac{h_t^2}{(4\pi )^2}\frac{1}{24}\left[ \left( 1 + \frac{1}{2}\frac{g^2c_{2\b} }{h_t^2} \right) - \frac{4}{5}\frac{X_t^2}{\mt^2} \right]\)  \\
%
  \(c_{WW}^{}\) &\(=\)& \(\frac{h_t^2}{(4\pi)^2} \frac{1}{16} \left[ \left( 1 - \frac{1}{6}\frac{g'^2c_{2\b} }{h_t^2} \right) - \frac{2}{5}\frac{X_t^2}{\mt^2} \right]\) &
  \(c_W^{}\) &\(=\)& \(\frac{h_t^2}{(4\pi)^2}\frac{1}{40} \frac{X_t^2}{\mt^2}\) \\
%
  \(c_{BB}^{}\) &\(=\)& \(\frac{h_t^2}{(4\pi)^2} \frac{17}{144} \left[ \left( 1 + \frac{31}{102}\frac{g'^2c_{2\b} }{h_t^2} \right) - \frac{38}{85}\frac{X_t^2}{\mt^2} \right]\) &
  \(c_B^{}\) &\(=\)& \(\frac{h_t^2}{(4\pi)^2}\frac{1}{40} \frac{X_t^2}{\mt^2}\) \\[.2cm]
  \hline
\end{tabular}
}
};
\end{scope}

%%%%%%%%%%%%% Higgs operators
\begin{scope}[xshift=.9cm,yshift = -3.4cm]
\node[anchor=west] at (0,0) {
\scalebox{1.1}{
\begin{tabular}{|rcl|}
  \hline
  \(c_H^{}\) &\(=\)& \(\frac{h_t^4}{(4\pi)^2}\frac{3}{4}\left[ \left( 1 + \frac{1}{3}\frac{g'^2c_{2\b} }{h_t^2} + \frac{1}{12} \frac{g'^4c_{2\b}^2}{h_t^4} \right) - \frac{7}{6}\frac{X_t^2}{\mt^2} \left( 1 + \frac{1}{14}\frac{(g^2 + 2g'^2)c_{2\b} }{h_t^2} \right) + \frac{7}{30}\frac{X_t^4}{\mt^2} \right]\) \\
%
  \(c_T^{}\) &\(=\)& \(\frac{h_t^4}{(4\pi )^2}\frac{1}{4}\left[ \left( 1 + \frac{1}{2}\frac{g^2c_{2\b} }{h_t^2} \right)^2 - \frac{1}{2}\frac{X_t^2}{\mt^2}\left( 1 + \frac{1}{2}\frac{g^2c_{2\b} }{h_t^2} \right) + \frac{1}{10}\frac{X_t^4}{\mt^4} \right]\) \\
%
  \(c_R^{}\) &\(=\)& \(\frac{h_t^4}{(4\pi)^2}\frac{1}{2}\left[ \left( 1 + \frac{1}{2}\frac{g^2c_{2\b}}{h_t^2} \right)^2 - \frac{3}{2}\frac{X_t^2}{\mt^2}\left( 1 + \frac{1}{12}\frac{(3g^2 + g'^2)c_{2\b}}{h_t^2} \right) + \frac{3}{10}\frac{X_t^4}{\mt^4} \right]\) \\
%
  \(c_D^{}\) &\(=\)& \(\frac{h_t^2}{(4\pi)^2}\frac{1}{20} \frac{X_t^2}{\mt^2}\) \\[0.2cm]
  \hline
\end{tabular}
}
};
\end{scope}

%%%%%%%%%%%%% c_6
\begin{scope}[xshift=-3.5cm,yshift = -6.4cm]
\node[anchor=west] at (0,0) {
\scalebox{1.1}{
\begin{tabular}{|rcl|}
  \hline
  \(c_6^{}\) &\(=\)& \(-\frac{h_t^6}{(4\pi )^2}\frac{1}{2}\left\{ \def\arraystretch{2.2} \begin{array}{l} \left[ 1 + \frac{1}{12}\frac{(3g^2 - g'^2)c_{2\beta }}{h_t^2} \right]^3 + \left[ - \frac{1}{12}\frac{(3g^2 + g'^2)c_{2\beta }}{h_t^2} \right]^3 + \left( 1 + \frac{1}{3}\frac{g'^2c_{2\beta }}{h_t^2} \right)^3 \\  - \frac{X_t^2}{\mt^2}\left[ 2\left( 1 + \frac{1}{12}\frac{(3g^2 - g'^2)c_{2\beta }}{h_t^2} \right) \left( 1 + \frac{1}{8}\frac{(g^2 + g'^2)c_{2\beta }}{h_t^2} \right) + \left(1 + \frac{1}{3}\frac{g'^2c_{2\beta }}{h_t^2} \right)^2 \right] + \frac{X_t^4}{\mt^4}\left[1 + \frac{1}{8}\frac{(g^2 + g'^2)c_{2\beta }}{h_t^2} \right] - \frac{X_t^6}{\mt^6}\frac{1}{10} \\ \end{array} \right\}\) \\
  \hline
\end{tabular}
}
};
\end{scope}

\end{tikzpicture}
%\end{table*}

